Naturalness of Attention: Revisiting Attention in Code Language Models

Language models for code such as CodeBERT offer the capability to learn advanced source code representation, but their opacity poses barriers to understanding of captured properties. Recent attention analysis studies provide initial interpretability insights by focusing solely on attention weights rather than considering the wider context modeling of Transformers. This study aims to shed some light on the previously ignored factors of the attention mechanism beyond the attention weights. We conduct an initial empirical study analyzing both attention distributions and transformed representations in CodeBERT. Across two programming languages, Java and Python, we find that the scaled transformation norms of the input better capture syntactic structure compared to attention weights alone. Our analysis reveals characterization of how CodeBERT embeds syntactic code properties. The findings demonstrate the importance of incorporating factors beyond just attention weights for rigorously understanding neural code models. This lays the groundwork for developing more interpretable models and effective uses of attention mechanisms in program analysis.

==> figures/z_mha_wo_mult.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{.95\columnwidth}
        \resizebox{\columnwidth}{!}{%
        $\displaystyle
        Z_{\text{MHA}} =
        \begin{bNiceMatrix}[right-margin = 6pt, left-margin = 6pt] 
        \text{z}_1[1,1] & \ldots & \text{z}_1[1,d'] & \text{z}_2[1,1] & \ldots & \text{z}_2[1,d']& \ldots &\text{z}_z[1,1] & \ldots & \text{z}_z[1,d'] \\  
        \text{z}_1[2,1] & \ldots & \text{z}_1[2,d'] & \text{z}_2[2,1] & \ldots & \text{z}_2[2,d'] & \ldots & \text{z}_z[2,1] & \ldots & \text{z}_z[2,d'] \\ 
        \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \ldots & \vdots \\
        \text{z}_1[n,1] & \ldots & \text{z}_1[n,d'] & \text{z}_2[n,1] & \ldots & \text{z}_2[n,d'] & \ldots & \text{z}_z[n,1] & \ldots & \text{z}_z[n,d'] \\ 
        \CodeAfter
            \tikz \node [fill=red!25, opacity=.2, draw, rounded corners, fit = (1-1) (last-3)] {} ; 
            \tikz \node [fill=green!25, opacity=.2, draw, rounded corners, fit = (1-4) (4-6)] { } ; 
            \tikz \node [fill=black!25, opacity=.2, draw, rounded corners, fit = (1-7) (last-7)] { } ;
            \tikz \node [fill=blue!25, opacity=.2, draw, rounded corners, fit = (1-8) (last-10)] { } ;
          \OverBrace[shorten,yshift=3mm]{1-1}{last-3}{\mathrm{z^{(1)}_{n\times d'}}}
          \OverBrace[shorten,yshift=3mm]{1-4}{last-6}{\mathrm{z^{(2)}_{n\times d'}}}
          \OverBrace[yshift=3mm]{1-7}{1-7}{...}
          \OverBrace[shorten,yshift=3mm]{1-8}{1-10}{\mathrm{z^{(h)}_{n\times d'}}}
        \end{bNiceMatrix}_{n \times hd'}
        $
        }
\end{subfigure}
~
\begin{subfigure}[t]{.7\columnwidth}
\resizebox{\columnwidth}{!}{%
$\displaystyle
W_{O} =
\begin{bNiceMatrix}[right-margin = 10pt, left-margin = 6pt] 
\text{w}[1,1] & \ldots &  \text{w}[1,d'] & \ldots & \text{w}[1,hd'] \\
\vdots & \vdots & \vdots & \vdots & \vdots  \\
\text{w}[d',1] & \ldots &  \text{w}[d',d'] & \ldots & \text{w}[d',hd'] \\
 &  &  &  &   \\
\text{w}[d'+1,1] & \ldots &  \text{w}[d'+1,d'] & \ldots & \text{w}[d'{+}1,hd'] \\
\vdots & \vdots & \vdots & \vdots & \vdots  \\
\text{w}[2d',1] & \ldots &  \text{w}[2d',d'] & \ldots & \text{w}[2d',hd'] \\
 &  &  &  &   \\
\vdots & \vdots & \vdots & \vdots & \vdots  \\
 &  &  &  &   \\
\text{w}[hd'{-}d',1] & \ldots &  \text{w}[hd'{-}d',d'] & \ldots & \text{w}[hd'{-}d',hd'] \\
\vdots & \vdots & \vdots & \vdots & \vdots  \\
\text{w}[hd',1] & \ldots &  \text{w}[hd',d'] & \ldots & \text{w}[hd',hd'] \\
\CodeAfter
\SubMatrix{\{}{1-1}{3-2}{.}[left-xshift=15pt, name=A] {}
\tikz \node [left] at (A-left.west) {$W_{O}^{(1)}$} ;
  \tikz \node [fill=red!25, opacity=.2, draw, rounded corners, fit = (1-1) (3-last.south east)] {} ; 
  \tikz \node [shift={(.1,0)}, fill=green!25, opacity=.2, draw, rounded corners, fit = (5-1) (7-last)] {} ;
  \tikz \node [fill=black!25, opacity=.2, draw, rounded corners, fit = (9-1) (9-last)] { } ;
  \tikz \node [shift={(-.15,0)}, fill=blue!25, inner sep=8pt, opacity=.2, draw, rounded corners, fit = (11-last) (13-1)] { } ;
  %\OverBrace[shorten,yshift=3mm]{1-1}{last-last}{\mathrm{h^{1}_{n\times d'}}}
\end{bNiceMatrix}_{hd' \times hd'}
$
}
\end{subfigure}
\caption{The result of concatenating each SA head's output, multiplied with the weight matrix, to calculate the final output of MHA. The highlighted blocks are the components that are attributed to each SA head.}
\label{fig:zmha_wo}
\end{figure*}

==> section/5_conclusion.tex <==
In this work, we have revisited the mathematical definition of Multihead Attention from prior works in natural language. We saw that it weighted sum of the transformation applied on the input sequence multiplied by the attention weight. This indicates that the properties code modelled is the product of not just one factor, but rather, of two. Future work involves assessing additional models, and languages given the diverse training techniques that were used in the former and the different properties of the latter. Unravelling the inner workings of neural code learners will grow increasingly important as representations advance.
